The 4/$\delta$ Bound: Designing Predictable LLM-Verifier Systems for Formal Method Guarantee

The integration of Formal Verification tools with Large Language Models (LLMs) offers a path to scale software verification beyond manual workflows. However, current methods remain unreliable: without a solid theoretical footing, the refinement process acts as a black box that may oscillate, loop, or diverge. This work bridges this critical gap by developing an LLM-Verifier Convergence Theorem, providing the first formal framework with provable guarantees for termination in multi-stage verification pipelines. We model the interaction not as a generic loop, but as a sequential absorbing Markov Chain comprising four essential engineering stages: \texttt{CodeGen}, \texttt{Compilation}, \texttt{InvariantSynth}, and \texttt{SMTSolving}. We prove that for any non-zero stage success probability ($\delta > 0$), the system reaches the \texttt{Verified} state almost surely. Furthermore, because of the sequential nature of the pipeline, we derive a precise latency bound of $\mathbb{E}[n] \leq 4/\delta$. We stress-tested this prediction in an extensive empirical campaign comprising over 90,000 trials. The results match the theory with striking consistency: every run reached verification, and the empirical convergence factor clustered tightly around $C_f\approx 1.0$, confirming that the $4/\delta$ bound accurately mirrors system behavior rather than serving as a loose buffer. Based on this data, we identify three distinct operating zones -- marginal, practical, and high-performance -- and propose a dynamic calibration strategy to handle parameter drift in real-world environments. Together, these contributions replace heuristic guesswork with a rigorous architectural foundation, enabling predictable resource planning and performance budgeting for safety-critical software.

==> sec_pretext.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PRE TEXT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section*{Statements and Declarations}

\subsection*{Conflict of Interest/Competing Interests}
The authors did not receive support from any organization for the submitted work.

\subsection*{Ethics Approval and Consent to Participate}
This study did not involve human participants or animal subjects, and therefore ethics approval and consent to participate are not applicable.

\subsection*{Consent for Publication}
Not applicable, as the manuscript does not contain any individual person's data in any form.

\subsection*{Data Availability}
This study did not generate or analyze any new datasets. 

\subsection*{Materials Availability}
No new physical or proprietary materials were created or used in this study. 

\subsection*{Code Availability}
To implement and validate this work, we developed a comprehensive simulation framework, available at \url{https://github.com/pierredantas}.

\subsection*{Author Contribution}
All authors contributed equally to the conceptualization, methodology, and writing of this work.

\newpage

